Large Language Model Guided Tree-of-Thought

In this paper, we introduce the Tree-of-Thought (ToT) framework, a novel approach aimed at improving the problem-solving capabilities of auto-regressive large language models (LLMs). The ToT technique is inspired by the human mind's approach for solving complex reasoning tasks through trial and error. In this process, the human mind explores the solution space through a tree-like thought process, allowing for backtracking when necessary. To implement ToT as a software system, we augment an LLM with additional modules including a prompter agent, a checker module, a memory module, and a ToT controller. In order to solve a given problem, these modules engage in a multi-round conversation with the LLM. The memory module records the conversation and state history of the problem solving process, which allows the system to backtrack to the previous steps of the thought-process and explore other directions from there. To verify the effectiveness of the proposed technique, we implemented a ToT-based solver for the Sudoku Puzzle. Experimental results show that the ToT framework can significantly increase the success rate of Sudoku puzzle solving. Our implementation of the ToT-based Sudoku solver is available on GitHub: \url{https://github.com/jieyilong/tree-of-thought-puzzle-solver}.

==> LLM Guided Tree-of-Thought - v0.1 - Arxiv/other.tex <==







\begin{itemize}
    \item MCTS Configuration 1. Trained solver + Rule-based scorer
    \item MCTS Configuration 2. Trained Solver + GPT4 API as a scorer
    \item MCTS Configuration 3. Trained Solver + Trained scorer
    \item MCTS Configuration 4. Teach ChatGPT to factor through prompt engineering, i.e. use ChatGPT as both the solver and scorer. 
    \item MCTS Configuration 5. Use ChatGPT as the solver + the Rule-based scorer
\end{itemize}

\begin{itemize}
    \item Pre-train an adversarial network using logical reasoning text corpus. Negative examples can be produced in mass 
    \item Auto-regressive LLMs as probabilistic models are good at pattern-recognition and pattern matching, e.g. to come up with a "solution framework",  or spark an idea, or suggest a certain theorem that could be useful, or point to a certain direction, since likely it saw these in similar problems it has seen. However, they are not good at accurate reasoning as of today.
    \item ``Tree-of-Thought'', or ToT for short. Note: ``tot'' has a meaning oa a very young child, which signifies this work as an very early exploration for automated logical reasoning leveraging language models. 
    \item Solver-Scorer network
    \item Special case: Let the model learn how to do factoring for multi-variable polynomials over finite fields. For this special case, we can develop a close-to-perfect reward model, i.e. Scorer. As a human solver, factoring typically requires tries and errors, which is a good testbed for tree-of-thought style of reasoning. Even though we have Bergkamp's algorithm which a solver can follow step-by-step, but we want to imitate human solver. \item There are different types of reasoning tasks. One with an algorithm which the model can follow step by step, e.g. multiplying two large integers together. And another type that requires trials and errors, e.g. solving challenging math questions. The former type of problem may be solvable by AR-LLM with token-by-token predictions, but ToT is more suitable for the latter type of tasks, where the solver knowns a set of ``tricks'' and needs to use these tricks creatively instead of following a prescribed algorithm to solve the problem. 
    \item LLMs + few shot + CoT is a special case of the new framework we propose.
    \item RL can explore much greater problem/solution spaces, which further improve the problem solving skills of the model, which is not unlike student enhances their understanding of the textbook by solving practicing problem sets.
    \item Future extensions: 1) Generic machine reasoning; 2) New math theorem discovery
    \item The rule-based scorer can be viewed as the model incorporating some rule-based knowledge into its own state.
    \item Reasoning requires "backtracking". If  "linear argument generation" can solve any reasoning task, then the model is essentially a non-deterministic Turing machine, which implies P = NP! By leveraging multi-round conversation with a persistent ``state'', we enable backtracking and enhance the forward-only LLM with ``long-term memory''.
    \item Our framework can be viewed as another option (aside from finetuning and prompt engineering) to extend or augment LLM to solve domain-specific tasks. LLM is used as a knowledge base, or an ideation engine.
    \item GPT seems to be good at ``short-range'' reasoning due to its probabilistic model nature. Couple it with an RL with state, it might be able to solve ``long-range'' reasoning tasks.
    \item the RL engine can encode ``rule-based'' model which can judge whether an intermediate solution violates any rules. This can be viewed a way to combine rules/knowledge with LLM. 
    \item the ``state'' can be viewed as the summary of the information accumulated over a long range of context, i.e. the ``long-term memory''. This way, we overcome the limitation on the max context length of the GPT/self-attention models.
\end{itemize}


==> other.tex <==







\begin{itemize}
    \item MCTS Configuration 1. Trained solver + Rule-based scorer
    \item MCTS Configuration 2. Trained Solver + GPT4 API as a scorer
    \item MCTS Configuration 3. Trained Solver + Trained scorer
    \item MCTS Configuration 4. Teach ChatGPT to factor through prompt engineering, i.e. use ChatGPT as both the solver and scorer. 
    \item MCTS Configuration 5. Use ChatGPT as the solver + the Rule-based scorer
\end{itemize}

\begin{itemize}
    \item Pre-train an adversarial network using logical reasoning text corpus. Negative examples can be produced in mass 
    \item Auto-regressive LLMs as probabilistic models are good at pattern-recognition and pattern matching, e.g. to come up with a "solution framework",  or spark an idea, or suggest a certain theorem that could be useful, or point to a certain direction, since likely it saw these in similar problems it has seen. However, they are not good at accurate reasoning as of today.
    \item ``Tree-of-Thought'', or ToT for short. Note: ``tot'' has a meaning oa a very young child, which signifies this work as an very early exploration for automated logical reasoning leveraging language models. 
    \item Solver-Scorer network
    \item Special case: Let the model learn how to do factoring for multi-variable polynomials over finite fields. For this special case, we can develop a close-to-perfect reward model, i.e. Scorer. As a human solver, factoring typically requires tries and errors, which is a good testbed for tree-of-thought style of reasoning. Even though we have Bergkamp's algorithm which a solver can follow step-by-step, but we want to imitate human solver. \item There are different types of reasoning tasks. One with an algorithm which the model can follow step by step, e.g. multiplying two large integers together. And another type that requires trials and errors, e.g. solving challenging math questions. The former type of problem may be solvable by AR-LLM with token-by-token predictions, but ToT is more suitable for the latter type of tasks, where the solver knowns a set of ``tricks'' and needs to use these tricks creatively instead of following a prescribed algorithm to solve the problem. 
    \item LLMs + few shot + CoT is a special case of the new framework we propose.
    \item RL can explore much greater problem/solution spaces, which further improve the problem solving skills of the model, which is not unlike student enhances their understanding of the textbook by solving practicing problem sets.
    \item Future extensions: 1) Generic machine reasoning; 2) New math theorem discovery
    \item The rule-based scorer can be viewed as the model incorporating some rule-based knowledge into its own state.
    \item Reasoning requires "backtracking". If  "linear argument generation" can solve any reasoning task, then the model is essentially a non-deterministic Turing machine, which implies P = NP! By leveraging multi-round conversation with a persistent ``state'', we enable backtracking and enhance the forward-only LLM with ``long-term memory''.
    \item Our framework can be viewed as another option (aside from finetuning and prompt engineering) to extend or augment LLM to solve domain-specific tasks. LLM is used as a knowledge base, or an ideation engine.
    \item GPT seems to be good at ``short-range'' reasoning due to its probabilistic model nature. Couple it with an RL with state, it might be able to solve ``long-range'' reasoning tasks.
    \item the RL engine can encode ``rule-based'' model which can judge whether an intermediate solution violates any rules. This can be viewed a way to combine rules/knowledge with LLM. 
    \item the ``state'' can be viewed as the summary of the information accumulated over a long range of context, i.e. the ``long-term memory''. This way, we overcome the limitation on the max context length of the GPT/self-attention models.
\end{itemize}

